Data-driven identification of latent port-Hamiltonian systems

Conventional physics-based modeling techniques involve high effort, e.g., time and expert knowledge, while data-driven methods often lack interpretability, structure, and sometimes reliability. To mitigate this, we present a data-driven system identification framework that derives models in the port-Hamiltonian (pH) formulation. This formulation is suitable for multi-physical systems while guaranteeing the useful system theoretical properties of passivity and stability. Our framework combines linear and nonlinear reduction with structured, physics-motivated system identification. In this process, high-dimensional state data obtained from possibly nonlinear systems serves as input for an autoencoder, which then performs two tasks: (i) nonlinearly transforming and (ii) reducing this data onto a low-dimensional latent space. In this space, a linear pH system, that satisfies the pH properties per construction, is parameterized by the weights of a neural network. The mathematical requirements are met by defining the pH matrices through Cholesky factorizations. The neural networks that define the coordinate transformation and the pH system are identified in a joint optimization process to match the dynamics observed in the data while defining a linear pH system in the latent space. The learned, low-dimensional pH system can describe even nonlinear systems and is rapidly computable due to its small size. The method is exemplified by a parametric mass-spring-damper and a nonlinear pendulum example, as well as the high-dimensional model of a disc brake with linear thermoelastic behavior.

==> fig/msd/matrices/matrices.tex <==
\pgfplotsset{
        % define the custom colormap
        colormap={gnuplot2}{
            rgb255=(0,0,0);
            rgb255=(0,0,4);
            rgb255=(0,0,8);
            rgb255=(0,0,12);
            rgb255=(0,0,16);
            rgb255=(0,0,20);
            rgb255=(0,0,24);
            rgb255=(0,0,28);
            rgb255=(0,0,32);
            rgb255=(0,0,36);
            rgb255=(0,0,40);
            rgb255=(0,0,44);
            rgb255=(0,0,48);
            rgb255=(0,0,52);
            rgb255=(0,0,56);
            rgb255=(0,0,60);
            rgb255=(0,0,64);
            rgb255=(0,0,68);
            rgb255=(0,0,72);
            rgb255=(0,0,76);
            rgb255=(0,0,80);
            rgb255=(0,0,84);
            rgb255=(0,0,88);
            rgb255=(0,0,92);
            rgb255=(0,0,96);
            rgb255=(0,0,100);
            rgb255=(0,0,104);
            rgb255=(0,0,108);
            rgb255=(0,0,112);
            rgb255=(0,0,116);
            rgb255=(0,0,120);
            rgb255=(0,0,124);
            rgb255=(0,0,128);
            rgb255=(0,0,131);
            rgb255=(0,0,136);
            rgb255=(0,0,140);
            rgb255=(0,0,144);
            rgb255=(0,0,147);
            rgb255=(0,0,152);
            rgb255=(0,0,156);
            rgb255=(0,0,160);
            rgb255=(0,0,163);
            rgb255=(0,0,168);
            rgb255=(0,0,172);
            rgb255=(0,0,176);
            rgb255=(0,0,179);
            rgb255=(0,0,184);
            rgb255=(0,0,188);
            rgb255=(0,0,192);
            rgb255=(0,0,195);
            rgb255=(0,0,200);
            rgb255=(0,0,204);
            rgb255=(0,0,208);
            rgb255=(0,0,211);
            rgb255=(0,0,216);
            rgb255=(0,0,220);
            rgb255=(0,0,224);
            rgb255=(0,0,227);
            rgb255=(0,0,232);
            rgb255=(0,0,236);
            rgb255=(0,0,240);
            rgb255=(0,0,243);
            rgb255=(0,0,248);
            rgb255=(0,0,252);
            rgb255=(0,0,255);
            rgb255=(3,0,255);
            rgb255=(7,0,255);
            rgb255=(10,0,255);
            rgb255=(13,0,255);
            rgb255=(16,0,255);
            rgb255=(19,0,255);
            rgb255=(22,0,255);
            rgb255=(25,0,255);
            rgb255=(28,0,255);
            rgb255=(32,0,255);
            rgb255=(35,0,255);
            rgb255=(38,0,255);
            rgb255=(41,0,255);
            rgb255=(44,0,255);
            rgb255=(47,0,255);
            rgb255=(50,0,255);
            rgb255=(53,0,255);
            rgb255=(57,0,255);
            rgb255=(60,0,255);
            rgb255=(63,0,255);
            rgb255=(66,0,255);
            rgb255=(69,0,255);
            rgb255=(72,0,255);
            rgb255=(75,0,255);
            rgb255=(78,0,255);
            rgb255=(82,0,255);
            rgb255=(85,0,255);
            rgb255=(88,0,255);
            rgb255=(91,0,255);
            rgb255=(94,0,255);
            rgb255=(97,0,255);
            rgb255=(100,0,255);
            rgb255=(103,0,255);
            rgb255=(107,0,255);
            rgb255=(110,0,255);
            rgb255=(113,0,255);
            rgb255=(116,0,255);
            rgb255=(119,0,255);
            rgb255=(122,0,255);
            rgb255=(125,0,255);
            rgb255=(128,0,255);
            rgb255=(132,0,255);
            rgb255=(135,0,255);
            rgb255=(138,1,253);
            rgb255=(141,3,251);
            rgb255=(144,5,249);
            rgb255=(147,7,247);
            rgb255=(150,9,245);
            rgb255=(153,11,243);
            rgb255=(157,13,241);
            rgb255=(160,15,239);
            rgb255=(163,17,237);
            rgb255=(166,19,235);
            rgb255=(169,21,233);
            rgb255=(172,23,231);
            rgb255=(175,25,229);
            rgb255=(178,27,227);
            rgb255=(182,29,225);
            rgb255=(185,31,223);
            rgb255=(188,33,221);
            rgb255=(191,35,219);
            rgb255=(194,37,217);
            rgb255=(197,39,215);
            rgb255=(200,41,213);
            rgb255=(203,43,211);
            rgb255=(207,45,209);
            rgb255=(210,47,207);
            rgb255=(213,49,205);
            rgb255=(216,51,203);
            rgb255=(219,53,201);
            rgb255=(222,55,199);
            rgb255=(225,57,197);
            rgb255=(228,59,195);
            rgb255=(232,61,193);
            rgb255=(235,63,191);
            rgb255=(238,65,189);
            rgb255=(241,67,187);
            rgb255=(244,69,185);
            rgb255=(247,71,183);
            rgb255=(250,73,181);
            rgb255=(253,75,179);
            rgb255=(255,77,177);
            rgb255=(255,79,175);
            rgb255=(255,81,173);
            rgb255=(255,83,171);
            rgb255=(255,85,169);
            rgb255=(255,87,167);
            rgb255=(255,89,165);
            rgb255=(255,91,163);
            rgb255=(255,93,161);
            rgb255=(255,95,159);
            rgb255=(255,97,157);
            rgb255=(255,99,155);
            rgb255=(255,101,153);
            rgb255=(255,103,151);
            rgb255=(255,105,149);
            rgb255=(255,107,147);
            rgb255=(255,109,145);
            rgb255=(255,111,143);
            rgb255=(255,113,141);
            rgb255=(255,115,139);
            rgb255=(255,117,137);
            rgb255=(255,119,135);
            rgb255=(255,121,133);
            rgb255=(255,123,131);
            rgb255=(255,125,129);
            rgb255=(255,127,127);
            rgb255=(255,129,125);
            rgb255=(255,131,123);
            rgb255=(255,133,121);
            rgb255=(255,135,119);
            rgb255=(255,137,117);
            rgb255=(255,139,115);
            rgb255=(255,141,113);
            rgb255=(255,143,111);
            rgb255=(255,145,109);
            rgb255=(255,147,107);
            rgb255=(255,149,105);
            rgb255=(255,151,103);
            rgb255=(255,153,101);
            rgb255=(255,155,99);
            rgb255=(255,157,97);
            rgb255=(255,159,95);
            rgb255=(255,161,93);
            rgb255=(255,163,91);
            rgb255=(255,165,89);
            rgb255=(255,167,87);
            rgb255=(255,169,85);
            rgb255=(255,171,83);
            rgb255=(255,173,81);
            rgb255=(255,175,79);
            rgb255=(255,177,77);
            rgb255=(255,179,75);
            rgb255=(255,181,73);
            rgb255=(255,183,71);
            rgb255=(255,185,69);
            rgb255=(255,187,67);
            rgb255=(255,189,65);
            rgb255=(255,191,63);
            rgb255=(255,193,61);
            rgb255=(255,195,59);
            rgb255=(255,197,57);
            rgb255=(255,199,55);
            rgb255=(255,201,53);
            rgb255=(255,203,51);
            rgb255=(255,205,49);
            rgb255=(255,207,47);
            rgb255=(255,209,45);
            rgb255=(255,211,43);
            rgb255=(255,213,41);
            rgb255=(255,215,39);
            rgb255=(255,217,37);
            rgb255=(255,219,35);
            rgb255=(255,221,33);
            rgb255=(255,223,31);
            rgb255=(255,225,29);
            rgb255=(255,227,27);
            rgb255=(255,229,25);
            rgb255=(255,231,23);
            rgb255=(255,233,21);
            rgb255=(255,235,19);
            rgb255=(255,237,17);
            rgb255=(255,239,15);
            rgb255=(255,241,13);
            rgb255=(255,243,11);
            rgb255=(255,245,9);
            rgb255=(255,247,7);
            rgb255=(255,249,5);
            rgb255=(255,251,3);
            rgb255=(255,253,1);
            rgb255=(255,255,4);
            rgb255=(255,255,17);
            rgb255=(255,255,29);
            rgb255=(255,255,42);
            rgb255=(255,255,54);
            rgb255=(255,255,67);
            rgb255=(255,255,79);
            rgb255=(255,255,92);
            rgb255=(255,255,104);
            rgb255=(255,255,117);
            rgb255=(255,255,130);
            rgb255=(255,255,142);
            rgb255=(255,255,154);
            rgb255=(255,255,167);
            rgb255=(255,255,179);
            rgb255=(255,255,192);
            rgb255=(255,255,204);
            rgb255=(255,255,217);
            rgb255=(255,255,230);
            rgb255=(255,255,242);
            rgb255=(255,255,255);
        },
    }
\fboxsep=00mm%padding thickness
\fboxrule=1pt%border thickness
\begin{tikzpicture}
    \pgfmathtruncatemacro{\ntest}{4}
    %% GROUND TRUTH
    % J
    \matrix [right=1ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] (J0) 
        {
            \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/J_ref_0.png}} \\
        };
    \foreach \i in {1,...,\ntest} 
        {
            \pgfmathtruncatemacro{\j}{\i-1}
            \matrix [matrix of math nodes, left delimiter={[}, right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (J\j.south west) (J\i) 
            {   
                \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/J_ref_\i.png}} \\
            };
        }
    \node[left=1ex] at (J\ntest.west) (J) {$\phJ=$};
    % R 
    \matrix [right=14ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (J0.east) (R0) 
        {
            \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/R_ref_0.png}} \\
        };
    \foreach \i in {1,...,\ntest} 
        {
            \pgfmathtruncatemacro{\j}{\i-1}
            \matrix [matrix of math nodes, left delimiter={[}, right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (R\j.south west) (R\i) 
            {
                \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/R_ref_\i.png}} \\
            };
        }
    \node[left=1ex] at (R\ntest.west) (R) {$\phR=$};
    % B 
    \matrix [right=14ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (R0.east) (B0) 
        {
            \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/B_ref_0}} \\
        };
    \foreach \i in {1,...,\ntest} 
        {
            \pgfmathtruncatemacro{\j}{\i-1}
            \matrix [matrix of math nodes, left delimiter={[}, right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at ($(B\j.south west)+(-1.5ex, 0)$) (B\i) 
            {
                \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/B_ref_\i.png}} \\
            };
        }
    \node[left=1ex] at (B\ntest.west) (B) {$\phB=$};
    %  %% IDENTIFIED
    % J
    \matrix [below=\ntest*4ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt]  at (J0.south) (Jid0) 
        {
            \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/J_pred_0.png}} \\
        };
    \foreach \i in {1,...,\ntest} 
        {
            \pgfmathtruncatemacro{\j}{\i-1}
            \matrix [matrix of math nodes, left delimiter={[}, right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (Jid\j.south west) (Jid\i) 
            {
                \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/J_pred_\i.png}} \\
            };
        }
    \node[left=1ex] at (Jid\ntest.west) (Jid) {$\phJ_{\Weights}=$};
    % R 
    \matrix [right=14ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (Jid0.east) (Rid0) 
        {
            \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/R_pred_0.png}} \\
        };
    \foreach \i in {1,...,\ntest} 
        {
            \pgfmathtruncatemacro{\j}{\i-1}
            \matrix [matrix of math nodes, left delimiter={[}, right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (Rid\j.south west) (Rid\i) 
            {
                \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/R_pred_\i.png}} \\
            };
        }
    \node[left=1ex] at (Rid\ntest.west) (Rid) {$\phR_{\Weights}=$};
    % B 
    \matrix [right=14ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (Rid0.east) (Bid0) 
        {
            \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/B_pred_0}} \\
        };
    \foreach \i in {1,...,\ntest} 
        {
            \pgfmathtruncatemacro{\j}{\i-1}
            \matrix [matrix of math nodes, left delimiter={[}, right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at ($(Bid\j.south west)+(-1.5ex, 0)$) (Bid\i) 
            {
                \fcolorbox{white}{red}{\includegraphics[height=1cm]{fig/msd/matrices/B_pred_\i.png}} \\
            };
        }
    \node[left=1ex] at (Bid\ntest.west) (Bid) {$\phB_{\Weights}=$};
    %% ERROR
    % J
   %  \node[below=5ex, anchor=north east] at (Jid.south east) (Je) {$\error_{\phJ}=$};
   %  \matrix [right=1ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (Je.east) (J2e) 
   %      {
   %          \includegraphics[height=1cm]{fig/msd/matrices/J_error_-0.394_0.394.png} \\
   %      };
   %  % R 
   % \node[below=5ex, anchor=north east] at (Rid.south east) (Re) {$\error_{\phR}=$};
   %  \matrix [right=1ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (Re.east) (R2e) 
   %      {
   %          \includegraphics[height=1cm]{fig/msd/matrices/R_error_-0.094_0.204.png} \\
   %      };
   %  % B 
   % \node[below=5ex, anchor=north east] at (Bid.south east) (Be) {$\error_{\phB}=$};
   %  \matrix [right=1ex, matrix of math nodes,left delimiter={[},right delimiter={]}, inner xsep=-2pt, inner ysep=0.25pt] at (Be.east) (B2e) 
   %      {
   %          \includegraphics[height=1cm]{fig/msd/matrices/B_error_-0.196_0.448.png} \\
   %      };
    \begin{axis}[
        hide axis,  % Hide the axis
        scale only axis,
        height=0.2cm,  % Adjust the height as needed
        width=2cm,  % Adjust the width as needed
        colorbar horizontal,     % Add colorbar
        colormap name=gnuplot2,
        colorbar style={
            at={($(Jid\ntest.south)+(0, 0ex)$)}, % Adjust the position relative to the TikZ node
            anchor=north, % Adjust the anchor point
        },
        point meta min=-2.9,  % Set the minimum value for the colorbar
        point meta max=2.9,  % Set the maximum value for the colorbar
    ]
        % Dummy plot to define the color range
        \addplot [draw=none] coordinates {(0,0) (1,1)};
    \end{axis}

    \begin{axis}[
        hide axis,  % Hide the axis
        scale only axis,
        height=0.2cm,  % Adjust the height as needed
        width=2cm,  % Adjust the width as needed
        colorbar horizontal,     % Add colorbar
        colormap name=gnuplot2,
        colorbar style={
            at={($(Rid\ntest.south)+(0, 0)$)}, % Adjust the position relative to the TikZ node
            anchor=north, % Adjust the anchor point
        },
        point meta min=-0.23,  % Set the minimum value for the colorbar
        point meta max=0.803,  % Set the maximum value for the colorbar
    ]
        % Dummy plot to define the color range
        \addplot [draw=none] coordinates {(0,0) (1,1)};
    \end{axis}
    
    \begin{axis}[
        hide axis,  % Hide the axis
        scale only axis,
        height=0.2cm,  % Adjust the height as needed
        width=2cm,  % Adjust the width as needed
        colorbar horizontal,     % Add colorbar
        colormap name=gnuplot2,
        colorbar style={
            at={($(Bid\ntest.south)+(0, 0)$)}, % Adjust the position relative to the TikZ node
            anchor=north, % Adjust the anchor point
        },
        point meta min=-0.31,  % Set the minimum value for the colorbar
        point meta max=1.446,  % Set the maximum value for the colorbar
    ]
        % Dummy plot to define the color range
        \addplot [draw=none] coordinates {(0,0) (1,1)};
    \end{axis}
\end{tikzpicture}
